Unsupervised Motion Representation Learning with Capsule Autoencoders

We propose the Motion Capsule Autoencoder (MCAE), which addresses a key challenge in the unsupervised learning of motion representations: transformation invariance. MCAE models motion in a two-level hierarchy. In the lower level, a spatio-temporal motion signal is divided into short, local, and semantic-agnostic snippets. In the higher level, the snippets are aggregated to form full-length semantic-aware segments. For both levels, we represent motion with a set of learned transformation invariant templates and the corresponding geometric transformations by using capsule autoencoders of a novel design. This leads to a robust and efficient encoding of viewpoint changes. MCAE is evaluated on a novel Trajectory20 motion dataset and various real-world skeleton-based human action datasets. Notably, it achieves better results than baselines on Trajectory20 with considerably fewer parameters and state-of-the-art performance on the unsupervised skeleton-based action recognition task.

==> sec_biography.tex <==





==> sec_broader_impact.tex <==
\section{Ethical Concerns}

Motion analysis techniques are in the foreground of the misuse of machine learning methods, among which adverse societal impacts and privacy breach are two major concerns.
Regarding the societal impacts, admittedly, our method has both upside and downside.
On one hand, a disentangled motion representation enables us better decode the information implicit in the trajectory, which has applications for example in ethology.
On the other hand, it could also be misused in mass surveillance.
Similar to other action analysis methods, if not well regulated, the downside risk could be enormous.
To prevent potential malicious applications, we need to establish appropriate boundaries of use and conduct ethical review when our method is applied to real-world applications.
Regarding the privacy concerns, our method is a step forward in privacy-preserving video analysis where it isolates motion information from the visual features.
If the vendors are prohibited to access the raw data and only given the motion representations, the subjects' sensitive information, such as gender and race, are preserved.
For a broader impact, we release the software and datasets of our research to the public.

==> sec_checklist.tex <==
\section*{Checklist}


\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{Please see \secref{sec:intro}.}
  \item Did you describe the limitations of your work?
    \answerYes{}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{Please check \secref{sec:conclusion}.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerNo{The source code and dataset will be released with the publication of the paper. Implementation details are covered in the supplementary material.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{Training details are mostly provided in \secref{sec:experiment} while some extra information is in the supplementary material.}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{We provided error bar on our T20 dataset. For experiments on NW-UCLA, NTURGBD-60, and NTURGBD-120, we followed the protocol in prior works.}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{Please see the first paragraph of \secref{sec:experiment}.}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{We used the publicly available NTURGBD60/120 and NW-UCLA dataset. The original papers have been cited.}
  \item Did you mention the license of the assets?
    \answerNA{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNo{The T20 dataset will be released with the publication of the paper.}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerYes{The data is publicly available and the consent has been described in the published paper.}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{No such information was found in the dataset we use.}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{No crowdsourcing research was conducted.}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}
